TiGDistill-BEV: Multi-view BEV 3D Object Detection via Target Inner-Geometry Learning Distillation

Accurate multi-view 3D object detection is essential for applications such as autonomous driving. Researchers have consistently aimed to leverage LiDAR's precise spatial information to enhance camera-based detectors through methods like depth supervision and bird-eye-view (BEV) feature distillation. However, existing approaches often face challenges due to the inherent differences between LiDAR and camera data representations. In this paper, we introduce the TiGDistill-BEV, a novel approach that effectively bridges this gap by leveraging the strengths of both sensors. Our method distills knowledge from diverse modalities(e.g., LiDAR) as the teacher model to a camera-based student detector, utilizing the Target Inner-Geometry learning scheme to enhance camera-based BEV detectors through both depth and BEV features by leveraging diverse modalities. Specially, we propose two key modules: an inner-depth supervision module to learn the low-level relative depth relations within objects which equips detectors with a deeper understanding of object-level spatial structures, and an inner-feature BEV distillation module to transfer high-level semantics of different key points within foreground targets. To further alleviate the domain gap, we incorporate both inter-channel and inter-keypoint distillation to model feature similarity. Extensive experiments on the nuScenes benchmark demonstrate that TiGDistill-BEV significantly boosts camera-based only detectors achieving a state-of-the-art with 62.8% NDS and surpassing previous methods by a significant margin. The codes is available at: https://github.com/Public-BOTs/TiGDistill-BEV.git.

==> tables/diffsetup_ablation.tex <==

% \begin{table*}[!t]
% \centering
% %\vspace{-0.2cm}
% % \resizebox{1\columnwidth}{!}
% {
% % \tablestyle{10pt}{1.0}
% \begin{tabular}{c|c|c|c|cc}

% \toprule
%           Backbone&Resolution&Multi-frame&Method& mAP&NDS  \\
%           \midrule
%           VoxelNet & - & \checkmark&Teacher & 0.564 & 0.646 \\\midrule
%           \multirow{4}{*}{ResNet-18}&\multirow{4}{*}{$256\times 704$}&\multirow{2}{*}{\checkmark}&Student & 0.285 & 0.405 \\ 
%               & & &  + TiG-BEV& \textbf{0.323 (\textcolor{blue}{+3.8\%})}         & \textbf{0.430 (\textcolor{blue}{+2.5\%})} \\
%               \cmidrule(lr){3-6}
%                 & & &  Student& 0.260  & 0.295 \\
%                & & &    + TiG-BEV& \textbf{0.294 (\textcolor{blue}{+3.4\%})}  & \textbf{0.335 (\textcolor{blue}{+4.0\%})}\\
%           \midrule
%          \multirow{4}{*}{ResNet-50}&\multirow{4}{*}{$256\times 704$}&\multirow{2}{*}{\checkmark}&Student & 0.329 & 0.431 \\ 
%               & & &    + TiG-BEV& \textbf{0.366 (\textcolor{blue}{+3.7\%})}         & \textbf{0.461 (\textcolor{blue}{+3.0\%})} \\
%               \cmidrule(lr){3-6}
              
%               & & &  Student& 0.298  & 0.328 \\
%                & & &  + TiG-BEV& \textbf{0.338 (\textcolor{blue}{+4.0\%})}  & \textbf{0.375 (\textcolor{blue}{+4.7\%})}\\
%           \midrule
%           \multirow{4}{*}{ResNet-101}&\multirow{4}{*}{$512\times 1408$}&\multirow{2}{*}{\checkmark}&Student & 0.393 & 0.487 \\ 
%               & & &  + TiG-BEV& \textbf{0.430 (\textcolor{blue}{+3.7\%})}         & \textbf{0.514 (\textcolor{blue}{+2.7\%})} \\
%               \cmidrule(lr){3-6}
%               & & &  Student& 0.345 & 0.366 \\
%                & & &    + TiG-BEV& \textbf{0.403 (\textcolor{blue}{+5.8\%})}        & \textbf{0.416 (\textcolor{blue}{+5.0\%)}} 
%          \\
%                \bottomrule
%     \end{tabular}}
%     \caption{\textit{Ablation Study of Image Backbones and Temporal Information.} CenterPoint~\cite{b53} and BEVDepth~\cite{b7} are adopted as the teacher and student models.}
%     \label{tab:many_ablation}
% \end{table*}


